Rethinking Diversity in Deep Neural Network Testing

Motivated by the success of traditional software testing, numerous diversity measures have been proposed for testing deep neural networks (DNNs). In this study, we propose a shift in perspective, advocating for the consideration of DNN testing as directed testing problems rather than diversity-based testing tasks. We note that the objective of testing DNNs is specific and well-defined: identifying inputs that lead to misclassifications. Consequently, a more precise testing approach is to prioritize inputs with a higher potential to induce misclassifications, as opposed to emphasizing inputs that enhance "diversity." We derive six directed metrics for DNN testing. Furthermore, we conduct a careful analysis of the appropriate scope for each metric, as applying metrics beyond their intended scope could significantly diminish their effectiveness. Our evaluation demonstrates that (1) diversity metrics are particularly weak indicators for identifying buggy inputs resulting from small input perturbations, and (2) our directed metrics consistently outperform diversity metrics in revealing erroneous behaviors of DNNs across all scenarios.

==> 01_introduction.tex <==
\section{Introduction}
DL systems have demonstrated remarkable performance across various machine learning tasks and also revolutionized modern society~\citep{Krizhevsky_imagenetclassification,nlp_2013}. More recently, large language models~\citep{gpt} and stable diffusion models~\citep{diffusion} have shown impressive, or even superhuman capabilities on many generative tasks. Despite the wide application of DL systems nowadays, their decision process remains quite black-box and less explainable to humans, and they are also shown to be vulnerable to various bugs~\citep{szegedy2014intriguing,goodfellow2015explaining,debug}. With the wide deployment of DL systems, especially in some safety-critical applications, it is important to ensure the security and trustworthiness of those systems. However, DL systems are also software artifacts, thus amenable to SE approaches.
%\jc{somewhat disjoint to the following paragraph. Could we massage the first paragraph to be like: wide adoption of ML system, but buggy behaviors, hence motivating the necessity for ML "testing". By viewing ML model as a program/software (add citations) --> opens up opportunities to bring insights from already well-founded software testing to ML testing.}

Testing, one of the classical SE techniques, has been practiced for decades to detect erroneous behaviors of traditional software~\citep{fuzzing-cacm}. By serving numerous inputs to the programs, testing can expose bugs when the execution deviates from the specification. Moreover, the inputs can serve as concrete examples for developers to demonstrate the existence of defects and to debug the program. %Past experience from testing on traditional software suggests that testing can be useful for understanding and debugging DL systems. 

In this work, we focus on DNN classification models as the programs under testing, because DNN classification models are the canonical deep learning task~\citep{deep-learning}, and also the standard model for DL testing~\citep{goodfellow2015explaining,diversity-boosting,ATS,deepxplore,NC-meaningful}. DNN classification models are parameterized numerical programs, aiming to align the classification results with human visual semantics through proper parameterization, which is usually achieved by differentiable data training. Therefore, a major goal to test DNNs is to find violations of the alignment between visual semantics and the DNN classification judgment.

In traditional software testing, tools often employ the adaptive testing scenario: a repeated loop involving input mutation, program execution, and evaluation of fitness~\citep{afl,tofu}. Inputs with higher fitness scores are prioritized or given more mutation resources for the next loop iterations. The goal is to expose bugs fast and this fitness quantifies how likely an input can expose bugs. As a result, to design an effective testing framework, an important task is to create a good metric that can prioritize potential defective inputs. 
Motivated by the idea of adaptive testing, to extend its utility toward detecting DNN bugs, a natural question arises as follows:
% we ought to design an effective metric to measure the input faultiness.
%jc{was talking about traditional software testing, and suddenly jumps to DNN testing. We should have a few connecting sentences; like, bringing this idea to identifying inputs to trigger misbehaviors of DL models --> need answers for the following question.}
% As a result, our work aims to answer the following question: 
\begin{focusbox}
What is a good metric that can prioritize potential erroneous inputs for DNNs? %\jc{how about; What is a good metric that prioritizes the potential inputs to trigger bugs in DNNs?}
\end{focusbox}



%There are two types of testing frameworks: \emph{diversity}-based testing and \emph{directed} testing. 
%Diversity-based testing relies on the assumption that diversified tests can execute the program thoroughly, and often expose corner cases that are overlooked by developers. This methodology is suitable for general-purpose testing, where tools aim to expose as many bugs as possible~\citep{afl,fuzzing-cacm}. 
%On the other hand, the goal of directed testing is more specific; such as detecting a \emph{particular type of bug} rather than any bug. Driven by the specific goal, directed testing prioritizes inputs that are more potential to expose particular bugs rather than inputs that improve the ``diversity''~\citep{aflgo,tofu}. For example, standard fuzz testing prioritizes tests that trigger unseen coverage. However, if the tool is to identify concurrency errors, test executions that are close to the potential data-race code in the program should be considered more promising to expose concurrency bugs~\citep{Razzer}. 

In recent years, researchers have proposed methods to test DNNs. Many of them are motivated by traditional software testing practices, in particular, to encourage the diversity of inputs. One of the common diversity measures in software testing is code coverage of execution from the inputs~\citep{fuzzing-cacm}. Researchers were motivated by this measure and defined similar metrics for DNNs. They treated neurons as the basic computational components, similar to basic blocks in programs, and defined diversity metrics in terms of neuron activation patterns~\citep{deepxplore}, namely, \textit{Neuron Coverage} (NC). 
However, later works argued that NC is \emph{not} a meaningful metric~\citep{NC-meaningful}. 
Till these days, the usage of neuron activation diversity remains controversial: some recent works re-confirm that NC does not bring significant advantage~\citep{nc-person} while some others still design diversity metrics based on neuron activations~\citep{diversity-boosting}. %In fact, researchers have observed that only a sparse subset of neurons in a large network play critical roles for the functionality~\cite{lottery,skill-neuron}. Merely increasing the neuron activation diversity violates these observations and leads to unnatural inputs~\cite{NC-meaningful}.

\paragraph{Motivation} In recent testing works, the evaluation overlooked the case small additive noise can be applied to the inputs~\citep{diversity-boosting,ATS}. This scenario is natural to consider because minor additive distortions can arise in the sensor system and they are unnoticeable to humans. Moreover, the phenomenon that small additive distortions can lead to distinct judgments in DNN is widely recognized in the DL community, known as the adversarial examples~\citep{szegedy2014intriguing}. It has been a popular research topic in DL over the past few years and motivate numerous research works~\citep{pgd,goodfellow2015explaining}. Hence, testing works missing adversarial examples without rational justification would undermine their credibility.

%In this paper, we provide an answer to the above controversy by \jc{any idea? some good short summary of the first contribution point}.

In this work, we provide a new testing framework that addresses the case where both small additive noise and also other natural input transformations such as image rotation, shifts, and shearing ~\citep{ATS,shorten2019survey} can be applied to images. The rationale is that these input transformations would not change the human visual semantics. Contrary to existing works that design different diversity metrics for DNN testing, we argue that many DNN testing tasks in the literature~\citep{deepxplore,diversity-boosting} should be treated as directed testing tasks. Unlike diversity-based testing, which relies on the assumption that diversified tests can execute the program thoroughly and expose corner cases~\citep{afl,fuzzing-cacm}, directed testing aims to detect specific bugs. Driven by the specific goal, directed testing prioritizes inputs that are more potential to expose particular bugs rather than inputs that improve the ``diversity''~\citep{aflgo,tofu}. For example, standard fuzz testing prioritizes tests that trigger unseen coverage. However, if the tool is to identify concurrency errors, test executions that are close to the potential data-race code in the program should be considered more promising to expose concurrency bugs~\citep{Razzer}. %that are overlooked by developers. This methodology is suitable for general-purpose testing, where tools aim to expose as many bugs as possible~\citep{afl,fuzzing-cacm}. 
%On the other hand, the goal of directed testing is more specific; such as detecting a \emph{particular type of bug} rather than any bug. Driven by the specific goal, directed testing prioritizes inputs that are more potential to expose particular bugs rather than inputs that improve the ``diversity''~\citep{aflgo,tofu}. For example, standard fuzz testing prioritizes tests that trigger unseen coverage. However, if the tool is to identify concurrency errors, test executions that are close to the potential data-race code in the program should be considered more promising to expose concurrency bugs~\citep{Razzer}. 


We refer to these bugs under detection as \emph{functionality} bugs because these bugs violate the DNN functionality. 
Also, the mathematical semantics of DNNs are simple compared to traditional software, so one can quantify how likely one input is to change the DNN's functionality, and this provides a measure for testing. Therefore, test generation should be guided by this directed measure rather than a diversity measure.
%
Moreover, we suggest that the testing can be even accelerated by exploiting an intrinsic nature of DL systems: differentiability.
% one of the most fundamental features of DL systems is that they are differentiable.
The differentiability of DNNs allows us to derive fast and precise linear approximations in a small neighborhood using gradients. %\jc{a bit unclear to grasp how to utilize the differentiability to accelerate the testing, and what's the intuition of connecting PGD to our framework. Current writeup is like we are just putting a list of terminologies and deferring all explanations to future sections. It's good to at least put some brief intuition/insights in the intro} 
As we will explain, state-of-the-art $\ell_p$-adversarial attacks from DL literature, projected gradient descent (PGD)~\citep{pgd}, can also be categorized into our testing framework. Moreover, we provide a careful mathematical analysis of gradient-based methods, which validates these methods for $\ell_p$-transformations, but also \emph{casts doubt} on their applications to other types of transformations.

%Apart from testing over small input distortions, we also notice some other discrepancies between the practices in the SE and DL communities. Even though DL systems are also programs and many SE techniques can be applied, DL has also been studied extensively outside SE due to its capability and popularity. Many practices in both communities are similar at a high level but still different in many ways. We point out some of these gaps and hopefully, this work can help bridge some of the gaps.

To summarize, we make the following contributions:
\begin{itemize}%[label=(\roman*)]
\setlength\itemsep{0.2em}
    \item Novelty: We provide a novel conceptual framework for several DL testing tasks and input transformations, and demonstrate that some state-of-the-art DL practices are the natural consequences of this framework; while~\citet{NC-meaningful,nc-person} only refuted the application of neuron coverage, a specific diversity measure. %We believe that our work can help clarify the controversial DNN testing topic, i.e., NC maximization; and bridge the gaps between practices in the SE and DL communities. In fact, we point out that the NC maximization metric generates out-of-distribution (OOD) inputs using the DL glossary.
    \item Formality: We formalize the testing problem and carefully analyze the input transformations. In particular, we demonstrate that although small distortions and natural input transformations do not alter human judgment, they have distinct mathematical properties and should be addressed differently for testing purposes. We justify this distinction both theoretically and empirically. We are unaware of any existing works that have studied this distinction and believe that this careful treatment is necessary for testing. %However, they can all be addressed within our testing framework.
    
    \item Verifiability: We evaluate our claims over four datasets and three types of standard DNN architectures, and open source the code and dataset needed for the evaluation at \url{https://github.com/BendingUnit-22/directNNTest}. %~\footnote{Our implementations are anonymously available at \url{https://github.com/BendingUnit-22/directNNTest}}.
    %\item To instantiate our framework, we provide several concrete testing metrics with careful mathematical analysis. Our unified testing framework allows us to handle various types of input transformations, and past works were unable to. Moreover, our analysis validates the application of gradients on $\ell_p$-adversarial attacks but also calls for rigorous scrutiny of gradient methods on other types of input transformations.
    %\item We empirically validate our framework with several carefully designed experiments 
    %\footnote{Our implementations are anonymously available at \url{https://github.com/BendingUnit-22/directNNTest}.}. 
    Moreover, we also compare our framework with several diversity-based methods. The result shows that our metrics are more effective in exposing the functionality bugs among all settings, and also reveals that the diversity metrics are weak indicators for bugs under small additive perturbations. %\zw{...}
\end{itemize}

==> 01_introduction_jc.tex <==
\section{Introduction}
Deep learning (DL) systems have demonstrated remarkable performance across various machine learning tasks and also revolutionized modern society~\citep{Krizhevsky_imagenetclassification,nlp_2013}. More recently, large language models~\citep{gpt} and stable diffusion models~\citep{diffusion} have shown impressive, or even superhuman capabilities on many generative tasks. Despite the wide application of DL systems nowadays, their decision process remains quite black-box and less explainable to humans, and they are also shown to be vulnerable to various bugs~\citep{szegedy2014intriguing,goodfellow2015explaining,debug}. With the wide deployment of DL systems, especially in some safety-critical applications, it is important to ensure the security and trustworthiness of those systems. However, DL systems are also software artifacts, thus amenable to SE approaches.
%\jc{somewhat disjoint to the following paragraph. Could we massage the first paragraph to be like: wide adoption of ML system, but buggy behaviors, hence motivating the necessity for ML "testing". By viewing ML model as a program/software (add citations) --> opens up opportunities to bring insights from already well-founded software testing to ML testing.}

Testing, one of the classical SE techniques, has been practiced for decades to detect erroneous behaviors of traditional software~\citep{fuzzing-cacm}. By serving numerous inputs to the programs, testing can expose bugs when the execution deviates from the specification. Moreover, the inputs can serve as concrete examples for developers to demonstrate the existence of defects and to debug the program. %Past experience from testing on traditional software suggests that testing can be useful for understanding and debugging DL systems. 

In this work, we focus on DNN classification models as the programs under testing, because the DNN classification problem is the canonical DL task~\citep{deep-learning}, and also used in recent popular DL testing works~\citep{goodfellow2015explaining,diversity-boosting,ATS,deepxplore,NC-meaningful}. DNN classification models are parameterized numerical programs, aiming to align the classification results with human visual semantics, which is usually achieved by differentiable data training. Therefore, a major goal to test DNNs is to find violations of the alignment between visual semantics and the DNN classification judgment. Because it is usually very expensive to obtain tests and manually label them, inputs are often generated by visual-semantics preserving transformations, which augment existing inputs with transformations such as unnoticeable noise, image rotation, shifts, and shearing~\citep{szegedy2014intriguing,ATS,shorten2019survey}~(\cref{sec:dnn-test}). These transformations are similar to input mutations in traditional software testing.  %Researchers have proposed metamorphic testing~\citep{metamorphic} to address this test generation problem, which augments existing inputs with metamorphic relations.

In traditional software testing, tools often employ the adaptive testing scenario: a repeated loop involving input mutation, program execution, and evaluation of fitness~\citep{afl,tofu}. Inputs with higher fitness scores are prioritized or given more mutation resources for the next loop iterations. The goal is to expose bugs fast and this fitness quantifies how likely an input can expose bugs. As a result, to design an effective testing framework, an important task is to create a good metric that can prioritize potential defective inputs. 
Motivated by the idea of adaptive testing, to extend its utility toward detecting DNN bugs, a natural question arises as follows:
% we ought to design an effective metric to measure the input faultiness.
%jc{was talking about traditional software testing, and suddenly jumps to DNN testing. We should have a few connecting sentences; like, bringing this idea to identifying inputs to trigger misbehaviors of DL models --> need answers for the following question.}
% As a result, our work aims to answer the following question: 
%\jc{can we make this question appear earlier in the intro? }
\begin{focusbox}
What is a good metric that can prioritize potential erroneous inputs for DNNs? %\jc{how about; What is a good metric that prioritizes the potential inputs to trigger bugs in DNNs?}
\end{focusbox}



%There are two types of testing frameworks: \emph{diversity}-based testing and \emph{directed} testing. 
%Diversity-based testing relies on the assumption that diversified tests can execute the program thoroughly, and often expose corner cases that are overlooked by developers. This methodology is suitable for general-purpose testing, where tools aim to expose as many bugs as possible~\citep{afl,fuzzing-cacm}. 
%On the other hand, the goal of directed testing is more specific; such as detecting a \emph{particular type of bug} rather than any bug. Driven by the specific goal, directed testing prioritizes inputs that are more potential to expose particular bugs rather than inputs that improve the ``diversity''~\citep{aflgo,tofu}. For example, standard fuzz testing prioritizes tests that trigger unseen coverage. However, if the tool is to identify concurrency errors, test executions that are close to the potential data-race code in the program should be considered more promising to expose concurrency bugs~\citep{Razzer}. 

In recent years, researchers have proposed methods to test DNNs. Many of them are motivated by traditional software testing practices, in particular, to encourage the diversity of inputs. One of the common diversity measures in software testing is code coverage of execution from the inputs~\citep{fuzzing-cacm}~(\cref{sec:st}). Researchers were motivated by this measure and defined similar metrics for DNNs. They treated neurons as the basic computational components, similar to basic blocks in programs, and defined diversity metrics in terms of neuron activation patterns~\citep{deepxplore}, namely, \textit{Neuron Coverage} (NC). 
However, later works argued that NC is \emph{not} a meaningful metric: higher NC leads to fewer defects detected, less natural inputs, and more biased prediction preferences~\citep{NC-meaningful}.
Till these days, the usage of neuron activation diversity remains controversial: some recent works re-confirm that NC does not bring significant advantage~\citep{nc-person} while some others still design diversity metrics based on neuron activations~\citep{diversity-boosting}(\cref{sec:diverse-dnn-testing}). %In fact, researchers have observed that only a sparse subset of neurons in a large network play critical roles for the functionality~\cite{lottery,skill-neuron}. Merely increasing the neuron activation diversity violates these observations and leads to unnatural inputs~\cite{NC-meaningful}.

In recent testing works, the evaluation often overlooked the case small noise can be applied to the inputs~\citep{diversity-boosting,ATS}. This scenario is natural to consider because minor distortions can arise in the sensor system and they are unnoticeable to humans. Moreover, the phenomenon that small distortions can lead to distinct judgments in DNN is widely recognized in the DL community, known as the adversarial examples~\citep{szegedy2014intriguing}. It has been a popular research topic in DL over the past few years and inspired numerous impactful works, including generative adversarial network and stable diffusion models~\citep{goodfellow2015explaining,gan,diffusion}. Hence, testing works missing adversarial examples without rational justification would undermine their credibility.

%In this paper, we provide an answer to the above controversy by \jc{any idea? some good short summary of the first contribution point}.

In this work, we provide a new testing framework that can address not only natural input transformations such as image rotation and shifts~\citep{ATS,shorten2019survey} but also small noise, all of which do not change the visual semantics of images. Contrary to existing works that design diversity metrics for DNN testing, we argue that these DNN testing tasks in the literature~\citep{deepxplore,diversity-boosting} should be treated as directed testing tasks. Unlike diversity-based testing, which relies on the assumption that diversified tests can execute the program thoroughly and expose corner cases~\citep{afl,fuzzing-cacm}, directed testing aims to detect specific bugs (\cref{sec:direct}). Driven by the specific goal, directed testing prioritizes inputs that are more potential to expose particular bugs rather than inputs that improve ``diversity''~\citep{aflgo,tofu}. %For example, standard fuzz testing prioritizes tests that trigger unseen coverage. However, if the tool is to identify concurrency errors, test executions that are close to the potential data-race code in the program should be considered more promising to expose concurrency bugs~\citep{Razzer}. %that are overlooked by developers. This methodology is suitable for general-purpose testing, where tools aim to expose as many bugs as possible~\citep{afl,fuzzing-cacm}. 
%On the other hand, the goal of directed testing is more specific; such as detecting a \emph{particular type of bug} rather than any bug. Driven by the specific goal, directed testing prioritizes inputs that are more potential to expose particular bugs rather than inputs that improve the ``diversity''~\citep{aflgo,tofu}. For example, standard fuzz testing prioritizes tests that trigger unseen coverage. However, if the tool is to identify concurrency errors, test executions that are close to the potential data-race code in the program should be considered more promising to expose concurrency bugs~\citep{Razzer}. 


We refer to these DNN bugs under detection as \emph{functionality} bugs because these bugs violate the DNN functionality. Our framework is based on the observation that DNNs are specialized numerical programs with relatively simple mathematical semantics, 
%Also, the mathematical semantics of DNNs are simple compared to traditional software, 
so one can quantify how likely one input is to change the DNN's functionality, and this provides a measure for testing. Therefore, test generation should be guided by this directed measure rather than a diversity measure (\cref{sec:forward}).
%
Moreover, we suggest that the testing can be even accelerated by exploiting an intrinsic nature of DL systems: differentiability.
% one of the most fundamental features of DL systems is that they are differentiable.
The differentiability of DNNs allows us to derive fast and precise linear approximations in a small neighborhood using gradients. %\jc{a bit unclear to grasp how to utilize the differentiability to accelerate the testing, and what's the intuition of connecting PGD to our framework. Current writeup is like we are just putting a list of terminologies and deferring all explanations to future sections. It's good to at least put some brief intuition/insights in the intro} 
As we will explain, state-of-the-art $\ell_p$-adversarial attacks from DL literature, projected gradient descent (PGD)~\citep{pgd}, can also be categorized into our testing framework (\cref{sec:diff}). 

Moreover, we provide a careful analysis of the image transformations and show that even if they are under the umbrella term of visual semantics preserving transformations, their mathematical properties are quite different. Small noise induces minor pixel changes while other types of image transformations can modify the pixels significantly. This distinction has a further impact on the scope of testing methods. Our analysis validates gradient methods for the small-noise transformation, but also \emph{casts doubt} on their applications to other types of transformations (\cref{sec:grad}). % \jc{reference to existing works utilizing this gradient-based approach}

%mainly gradient-based methods, which validates these methods for $\ell_p$-transformations, but also \emph{casts doubt} on their applications to other types of transformations (\cref{sec:grad}).

%Apart from testing over small input distortions, we also notice some other discrepancies between the practices in the SE and DL communities. Even though DL systems are also programs and many SE techniques can be applied, DL has also been studied extensively outside SE due to its capability and popularity. Many practices in both communities are similar at a high level but still different in many ways. We point out some of these gaps and hopefully, this work can help bridge some of the gaps.

To summarize, we make the following contributions:
\begin{itemize}%[label=(\roman*)]
\setlength\itemsep{0.2em}
    \item Novelty: We provide a novel conceptual framework for DNN functionality testing, and demonstrate that some state-of-the-art DL practices are the natural consequences of this framework; while~\citet{NC-meaningful,nc-person} only refuted the application of neuron coverage, a specific diversity measure. Hence, we are more constructive compared to~\citet{NC-meaningful,nc-person}. %\jc{unclear why suddenly these two works are here for comparison of novelty}.%We believe that our work can help clarify the controversial DNN testing topic, i.e., NC maximization; and bridge the gaps between practices in the SE and DL communities. In fact, we point out that the NC maximization metric generates out-of-distribution (OOD) inputs using the DL glossary.
    \item Formality: We formalize the testing problem and carefully analyze the input transformations. In particular, we demonstrate that although small distortions and natural image transformations do not alter human judgment, they have distinct mathematical properties and should be addressed differently for testing purposes. We justify this distinction both theoretically and empirically. We are unaware of any existing works that have explicitly studied this distinction and believe that this careful treatment is necessary. %for testing. %However, they can all be addressed within our testing framework.
    
    \item Verifiability: We evaluate our claims over four datasets and three types of standard DNN architectures, and open source the code and dataset needed for the evaluation~\footnote{\url{https://github.com/BendingUnit-22/directNNTest}}. %~\footnote{Our implementations are anonymously available at \url{https://github.com/BendingUnit-22/directNNTest}}.
    %\item To instantiate our framework, we provide several concrete testing metrics with careful mathematical analysis. Our unified testing framework allows us to handle various types of input transformations, and past works were unable to. Moreover, our analysis validates the application of gradients on $\ell_p$-adversarial attacks but also calls for rigorous scrutiny of gradient methods on other types of input transformations.
    %\item We empirically validate our framework with several carefully designed experiments 
    %\footnote{Our implementations are anonymously available at \url{https://github.com/BendingUnit-22/directNNTest}.}. 
    Moreover, we also compare our framework with several diversity-based methods. The result shows that our metrics are more effective in exposing the functionality bugs among all settings, and also reveals that the diversity metrics are weak indicators for bugs induced by small input perturbations. %\zw{...}
\end{itemize}

==> 02_prelim.tex <==
\section{background}
\subsection{Mathematical Notations and Definitions}
Let $[n] = \{1,\ldots,n\}$. 
For a vector $v\in\R^n$, $\sign(v) \in \{-1, 0, 1\}^n$ such that 
\[ \sign(v)_i = \left\{ \begin{array}{ll}
            1, & \mbox{$v_i > 0$}\\
            0, & \mbox{$v_i = 0$}\\
            -1, & \mbox{$v_i < 0$}\end{array} \right. 
\]
$A^T$ denotes the transpose of a matrix $A$.
Let $\norm{v}_p$ denote the $\ell_p$ norm of a vector $v$: 
\[\norm{v}_p = \sqrt[\leftroot{-1}\uproot{8}\scriptstyle p]{\sum_{i=1}^n |v_i|^p}.\]
The canonical Euclidean norm is then $\norm{v}_2$, and another commonly considered norm on the input is the $\ell_\infty$-norm:
\[
\norm{v}_\infty = \max_{i\in[n]}{|v_i|}.
\]
For two functions $f$ and $g$, $f\func g(x) = f(g(x))$ denotes the composition of $f$ and $g$. If $f:\R^n\rightarrow \R$ is differentiable, we use $D^{i}f$ to denote the $i$-th order differentiation of partial derivatives, e.g., $D^{1}f$ is the gradient of $f$, and $D^{2}f$ is the Hessian of $f$. As a convention, we omit $1$ when we denote gradient, i.e., we use $Df$ to denote the gradient of $f$.

For an infinitely differentiable multivariate function $f:\R^n\rightarrow \R$, the Taylor expansion $T$ of $f$ at $a\in \R^n$ is
\[
T(a+\Delta x) = f(a)+(\Delta x)^TDf(a)+\frac{1}{2}(\Delta x)^TD^2f(a) (\Delta x)+\ldots,
\]
Therefore, $T(a+\Delta x)$ is an infinite series. If $f$ is analytic, then $T(a+\Delta x)$ converges to $f(a+\Delta x)$~\citep{babyrudin}. In this work, we only work with the first two terms of $T$, i.e., we only consider 
\begin{equation}\label{eq:linear}
    f(a)+(\Delta x)^TDf(a).
\end{equation}
Given the information of $f$ at $a$, i.e., $f(a)$ and $Df(a)$,~\cref{eq:linear} is the linear approximation of $f$ at $a+\Delta x$. This can provide an estimation of $f(a+\Delta x)$ if we do not want to evaluate $f$ at $a+\Delta x$ directly, i.e.,  $f(\Delta x+a)\approx f(a)+(\Delta x)^TDf(a)$.
\begin{remark}\label{rm:quality}
The quality of linear approximation depends on how large $x$ is, and how close $f$ is to a linear function.
\end{remark}
\subsection{Software Testing}\label{sec:st}
Large software artifacts have been an integral part of modern society for decades and are evolving on a constant basis. Despite its ubiquity, software usually contains various defects and some of them can raise serious security concerns. Testing remains one of the most efficient ways to demonstrate the presence of bugs. Since modern software is complicated, bugs can occur anywhere in the program. For example, a buffer usage in the program could potentially introduce overflow and a pointer operation could lead to a NULL pointer dereference. 

Due to the omnipresence of risky operations in the program, automated testing techniques are commonly guided by the diversity heuristics: a diverse set of inputs can execute the program thoroughly and therefore result in more bugs revealed~\citep{fuzzing-cacm}. One of the diversity measures in testing is code coverage, which can have multiple granularities such as function coverage, basic block coverage, and path coverage. For example, the famous fuzzing tool, American Fuzzy Lop (AFL) is a state-of-the-art general-purpose fuzzer that employs the coverage maximization heuristics~\citep{afl}. With a loop involving input
mutation, execution, and evaluation of coverage-based diversity metric, AFL generates inputs aiming to execute different parts of the program and has successfully detected numerous bugs in various applications.

\subsection{DNNs}
%In the last decade, neural networks have achieved unprecedented success in many machine learning tasks, and recently achieved even superhuman performances. %Even though DNNs are essentially a numerical program, its developing process differ Our methodology applies to all network architectures, and we will evaluate it on various network models. We briefly discuss other architectures after the discussion of the feed-forward network.
%However, the decision process of DNNs remains largely mysterious and DL systems are known vulnerable to various types of bugs. As a result, we would also want to test and debug DL systems. 
In this work, we mainly focus on feed-forward DNNs (convolutional neural networks are also a type of DNNs), because DNNs are the canonical DL architecture~\citep{deep-learning}. Here we discuss some basics of DNNs that are needed to elaborate our testing approach.

A feed-forward DNN $f:\R^m\rightarrow \R^l$ is a composition of affine transformations and non-linear activation functions:
\[
f_1(x)=  W^{(1)} x+b^{(1)};\; f_i(x)=  W^{(i)}\act(x)+b^{(i)}, i=2,\ldots,d.
\]
where $W^{(i)}\in \R^{n_{i+1}\times n_{i}}$ is the weight matrix between the layers, $n_1 = m$ and $n_{d+1}=l$, $d$ is the depth of the network, and $b^{(i)}\in \R^{n_{i+1}}$ is the bias term. $\act$, the activation, is an element-wise non-linear function. $f = f_d\func\cdots\func f_1$. 
\begin{remark}\label{rm:non-linear}
    In general, a neural network is highly non-linear. Therefore, for the linear approximation to be precise, we would need $\Delta x$ to be small in~\cref{eq:linear}.
\end{remark}

In this work, we only consider the standard classification tasks. $f: \R^m\rightarrow \R^l$ has $l$ outputs. Let $f^{(i)}$ be the $i$-th output of $f$. The classification of an input $x$ is $\class(f,x)=\argmax_{k\in[l]}f^{(k)}(x)$. Suppose that the prediction of $x$ is $i$, then $f^{(i)}(x)> f^{(j)}(x)$ for all $j\neq i$. The output of $f$ is called the logit score, and the classification model outputs the class with the highest logit score.

%One important difference between neural networks and traditional software is that neural networks are \emph{differentiable} numerical programs. This enables composing neural networks in a data-driven way. Unlike traditional software, where the logic is manually created by developers, the functionality of neural networks is decided by the weight matrices which are trained to fit the data rather than manually specified. This fitting process usually requires a loss to measure the difference between the functionality and ground truth and then minimizes the loss with variants of gradient descent, which is possible because the program is differentiable~\citep{deep-learning}. 

%%Apart from the standard data fitting, one can also modify the training process to achieve additional properties beyond clean accuracy, for example, robustness~\citep{pgd}. As we will demonstrate, we can also incorporate our framework to train models that are less prone to bugs.

Compared with traditional software, which might contain complicated structures like pointer aliasing, various data structures and indirect function calls,
DNNs are specialized numerical programs only involving a few operations: matrix addition and multiplication, activation function, and the max function. % with simple mathematical semantics. % (even though the decision process of DNNs is unclear to humans). 
Therefore, the techniques designed to handle the complexity in traditional software might not be directly applicable to DNNs. In particular, we want to point out that diversity-based methods in software testing are not the ideal testing framework for several DNN testing tasks.

\subsection{DNN Testing}\label{sec:dnn-test}
The functionality of DNNs is to classify inputs correctly aligned with human perception. Therefore, functionality bugs in the classifier setting should be incorrect classification, and the testing goal is to generate inputs that are misclassified. However, obtaining tests and manually labeling them is usually a very expensive process. Researchers have proposed metamorphic testing~\citep{metamorphic} to address this test generation problem, which augments existing inputs with metamorphic relations. %The metamorphic testing generates new inputs by transforming existing ones while preserving their labels. 
Because the functionality of vision models is to align the model judgment with human perception, one important metamorphic relation is \emph{equivalence-preserving} image transformations under the visual semantics.
Such transformations include small perturbations, image rotation, zooming, and brightness change and they do not change human judgment. We refer to these transformations as visual semantics-preserving transformations. They can augment the original dataset by applying those transformations on labeled inputs. If any of those transformed inputs can alter the DNN's prediction, then we identify misclassified inputs. In this work, we focus on identifying misclassified inputs, which we refer to as \emph{functionality testing}.
Rather than manually collected and labeled, these inputs are generated from a few compositions of small semantics-preserving transformations. Recent popular works can be categorized into functionality testing~\citep{diversity-boosting,deepxplore,szegedy2014intriguing,goodfellow2015explaining}, to change the DNN prediction by applying semantics-preserving transformations on the inputs. Small distortions are also known as adversarial examples in DL literature~\citep{szegedy2014intriguing,goodfellow2015explaining}.

\begin{remark}
  Even if small perturbations and natural image transformations are under the same umbrella term, visual semantics-preserving transformations, they are mathematically distinct transformations. Natural image transformations like image rotations can change the pixel representation of images significantly. 
\end{remark}

\subsection{Diversity in DNN Testing}\label{sec:diverse-dnn-testing}
Inspired by the success of traditional software testing, researchers have devised various diversity measures for DL system testing. One of the first diversity measures is NC~\citep{deepxplore}, similar to the code coverage in traditional software testing, which measures how many neurons are activated above a specified threshold $k$. The assumption is that the more neurons are activated, the more states of DNNs are explored. Later works refined the definition of NC and proposed several structural variants of NC, including the neuron boundary coverage and strong neuron activations~\citep{deep_gauge}. More recently,~\citep{diversity-boosting} proposed to use intermediate layer activation divergence between metamorphic inputs as an indicator to detect prediction violations, arguing that inputs with different intermediate activation patterns should also have divergent predictions.~\citep{ATS} proposed a measure to compute the fault pattern of inputs based on the normalized logit score, and a test selection algorithm that chooses a subset of inputs with diverse fault patterns and higher prediction uncertainty.

\subsection{Directed Software Testing}\label{sec:direct}
Unlike general-purpose software testing tools such as AFL, directed testing prioritizes inputs that are close to the specific testing goal. For example, a data-race testing tool should prioritize inputs that are more likely to trigger concurrency bugs rather than inputs with unseen coverage~\citep{Razzer}. In software testing, this proximity can often be measured statically by distance in code. For example, inputs that trigger concurrency bugs necessarily execute code where data race can occur, so the proximity can be measured by the distance between the execution trace and those race condition targets in the program. Mutating inputs close to those targets can generate inputs even closer to the targets and eventually reach the target and potentially trigger specific bugs~\citep{tofu}. 

Researchers have developed several directed testing tools, and shown that they are more capable of detecting specific bugs than general-purpose testing tools~\citep{aflgo}. In fact, we argue that DNN functionality testing should be considered as directed testing tasks conceptually, because bugs within these tasks are well-defined and specific.

==> abandon.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{p{3cm}p{1.9cm}p{1.0cm}p{1.05cm}p{1.1cm}p{1.0cm}p{1.0cm}p{1.2cm}p{1.2cm}p{1.0cm}}
\toprule
%\multicolumn{6}{c}{\centering Number of Correctly Classified Inputs} \\
%\midrule
\centering Data, Model, Accuracy & \hfil Transformations &\hfil Norm & \hfil BM\&BL & \hfil FM\&BM  & \hfil FL\&BL & \hfil FL\&BD & \hfil FL\&BD-F & \hfil FL\&ATS & FL\&NC  \\
\midrule
\hfil SVHN, & \hfil LP  & \hfil 0.20  & \hfil 0.86 & \hfil 0.92 & \hfil 0.86 & \hfil  0.52& \hfil 0.53 & \hfil 0.59 & \hfil 0.52 \\
\cmidrule{2-10}
\centering VGG, & \hfil Benign & \hfil 8.56 & \hfil 0.95& \hfil 0.62 & \hfil 0.59 &\hfil 0.72& \hfil 0.75 &\hfil 0.72  &\hfil 0.68\\
\cmidrule{2-10}
\hfil 95.49\% & \hfil Mixed  & \hfil 4.29  & \hfil 0.93 & \hfil 0.72  & \hfil  0.68 &\hfil 0.69& \hfil 0.70&\hfil 0.68 &\hfil 0.67\\
\midrule
\hfil SVHN, & \hfil LP  & \hfil 0.20  & \hfil 0.88& \hfil 0.94 & \hfil 0.89 & \cellcolor{yellow!60}\hfil       {0.40}& \cellcolor{yellow!60} \hfil       {0.41} &\hfil 0.59  & \cellcolor{yellow!60}\hfil       {0.40}  \\
\cmidrule{2-10}
\centering ResNet-9, & \hfil Benign & \hfil 8.56 & \hfil 0.95& \hfil 0.61 & \hfil 0.68 & \hfil 0.71& \hfil 0.75 &\hfil 0.74 &\hfil 0.68  \\
\cmidrule{2-10}
\hfil 95.51\% & \hfil Mixed  & \hfil 4.29  & \hfil 0.94 & \hfil 0.69 & \hfil 0.65 & \hfil 0.67& \hfil 0.69 &\hfil 0.70  &\hfil 0.65 \\
\midrule
\hfil CIFAR10, & \hfil LP  & \hfil 0.20  & \hfil 0.79& \hfil 0.87 & \hfil 0.74 &\cellcolor{yellow!60}\hfil       {0.49}&\cellcolor{yellow!60} \hfil       {0.50}&\hfil 0.56 &\cellcolor{yellow!60}\hfil       {0.48}\\
\cmidrule{2-10}
\centering VGG, & \hfil Benign & \hfil 11.34 & \hfil 0.96& \hfil 0.60 & \hfil 0.57 &\hfil 0.76& \hfil 0.81 &\hfil 0.74  &\hfil 0.71 \\
\cmidrule{2-10}
\hfil 91.26\% & \hfil Mixed  & \hfil 5.77  & \hfil 0.92 &\hfil 0.69 & \hfil 0.64 &\hfil 0.73& \hfil 0.76& \hfil 0.71 &\hfil 0.70\\
\midrule
\hfil CIFAR10, & \hfil LP  & \hfil 0.20  & \hfil 0.88& \hfil 0.92 & \hfil 0.87 &\cellcolor{yellow!60} \hfil       {0.46}& \cellcolor{yellow!60}\hfil      {0.47} &\hfil 0.60 &\hfil  \cellcolor{yellow!60}      {0.46} \\
\cmidrule{2-10}
\centering ResNet-9, & \hfil Benign & \hfil 11.34 & \hfil 0.95& \hfil 0.59 & \hfil 0.65 & \hfil 0.75& \hfil 0.77&\hfil 0.76  &\hfil 0.70 \\
\cmidrule{2-10}
\hfil 90.05\% & \hfil Mixed  & \hfil 5.77  & \hfil 0.95& \hfil 0.68 & \hfil 0.64& \hfil 0.73& \hfil 0.72 & \hfil 0.73& \hfil 0.69\\
\midrule
\hfil CIFAR100, & \hfil LP  & \hfil 0.20  & \hfil 0.85& \hfil 0.86 & \hfil 0.80 & \hfil 0.52& \hfil 0.52& \hfil-- & \hfil 0.52   \\
\cmidrule{2-10}
\centering VGG, & \hfil Benign & \hfil 11.59 & \hfil 0.96& \hfil 0.62 & \hfil 0.56  & \hfil 0.75& \hfil 0.75& \hfil--  & \hfil 0.69\\
\cmidrule{2-10}
\hfil 65.98\% & \hfil Mixed  & \hfil 5.89  & \hfil 0.94& \hfil 0.72 & \hfil 0.64& \hfil 0.72 & \hfil 0.72 & \hfil -- & \hfil 0.69\\
\midrule
\hfil CIFAR100, & \hfil LP  & \hfil 0.20  & \hfil 0.88& \hfil 0.88& \hfil 0.84 & \hfil 0.53 & \hfil 0.53& \hfil -- & \hfil 0.53 \\
\cmidrule{2-10}
\centering ResNet-18, & \hfil Benign & \hfil 11.59 & \hfil 0.97 & \hfil 0.63 & \hfil 0.57 & \hfil 0.74 & \hfil 0.75& \hfil --& \hfil 0.67\\
\cmidrule{2-10}
\hfil 66.23\% & \hfil Mixed  & \hfil 5.89  & \hfil 0.95 & \hfil 0.73 & \hfil 0.65 & \hfil 0.71 & \hfil 0.72& \hfil -- & \hfil  0.68\\
\bottomrule
\end{tabular}
\newline\newline 
\caption{Similarity measures (RBO) between ranked lists according to various prioritization metrics. The first column specifies the model, dataset and accuracy on the test dataset. The second column specifies what transformations are used for the experiment. The third column norm measures the average $\ell_2$-norm of all transformations. The rest of the columns measure the similarity between pairs of metric scores. We \colorbox{yellow!60}{highlight} cases where numbers stand for negative correlations.}\label{tab:rq1-c}
\end{center}
\end{table*}

%\subsection{Full Table 3}
\begin{table*}
\begin{center}
\begin{tabular}{p{5cm}p{1.9cm}p{1cm}p{1.2cm}p{1.3cm}p{1.2cm}p{1.2cm}}
\toprule
%\multicolumn{6}{c}{\centering Number of Correctly Classified Inputs} \\
%\midrule
\centering Data, Model, Accuracy, Transformations & \hfil Fitness &\hfil Iter 1 & \hfil Iter 2 & \hfil Iter 3  & \hfil Iter 4 & \hfil Iter 5  \\
\midrule
\hfil & \hfil FM & \hfil 96.37\% & \hfil 94.91\% & \hfil 92.91\% & \hfil 90.08\% & \hfil 86.65\% \\
\cmidrule{2-7}
\hfil & \hfil FL & \hfil 96.38\% & \hfil 95.01\% & \hfil 92.98\% & \hfil 90.34\% & \hfil 87.05\% \\
\cmidrule{2-7}
\hfil & \hfil BM  & \hfil 70.27\% & \hfil 15.5\% & \hfil 2.4\% & \hfil 0.2\% & \hfil 0.03\%  \\
\cmidrule{2-7}
\centering MNIST, & \hfil BL & \hfil 33.02\% & \hfil 0.65\% & \hfil 0.0\% & \hfil 0.0\% & \hfil 0.0\%  \\
\cmidrule{2-7}
\hfil LeNet-1, & \hfil BD & \hfil 97.4\% & \hfil 97.3\% & \hfil 97.26\% & \hfil 97.11\% & \hfil 96.95\%  \\
\cmidrule{2-7}
\hfil 97.32\% & \hfil BD-F & \hfil 97.21\% & \hfil 97.11\% & \hfil 97.04\% & \hfil 96.92\% & \hfil 96.6\% \\
\cmidrule{2-7}
\hfil LP & \hfil ATS & \hfil 32.69\% & \hfil 24.1\% & \hfil 21.63\% & \hfil 20.72\% & \hfil 20.33\% \\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil 97.28\% & \hfil 97.3\% & \hfil 97.27\% & \hfil 97.17\% & \hfil 97.22\% \\
\midrule
\hfil & \hfil FM & \hfil 94.94\%& \hfil 94.42\% & \hfil 93.89\% & \hfil 93.20\% & \hfil 92.56\%\\
\cmidrule{2-7}
\hfil & \hfil FL  & \hfil 94.94\%& \hfil 94.43\%& \hfil 93.84\%& \hfil 93.22\% & \hfil 92.54\% \\
\cmidrule{2-7}
\centering SVHN, & \hfil BM & \hfil 82.96\% & \hfil 62.08\% & \hfil 41.74\% & \hfil 26.44\% & \hfil 16.25\% \\
\cmidrule{2-7}
\centering ResNet-9, & \hfil BL & \cellcolor{yellow!60}\hfil 76.80\% & \cellcolor{yellow!60}\hfil 50.18\% & \cellcolor{yellow!60}\hfil 30.49\% & \cellcolor{yellow!60}\hfil 17.66\% & \cellcolor{yellow!60}\hfil 9.68\% \\
\cmidrule{2-7}
\hfil 95.51\% & \hfil BD & \hfil 95.49\%& \hfil 95.49\% & \hfil 95.48\% & \hfil 95.49\% & \hfil 95.47\%\\
\cmidrule{2-7}
\hfil LP & \hfil BD-F & \hfil 95.48\%& \hfil 95.42\% & \hfil 95.40\% & \hfil 95.38\% & \hfil 95.32\%\\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil 95.50\%& \hfil 95.50\% & \hfil 95.47\% & \hfil 95.42\% & \hfil 95.41\%\\
\midrule
\hfil & \hfil FM & \hfil 90.21\%& \hfil 89.16\% & \hfil 88.08\% & \hfil 86.96\% & \hfil 85.56\%\\
\cmidrule{2-7}
\hfil & \hfil FL  & \hfil 90.22\%& \hfil 89.17\%& \hfil 88.1\%& \hfil 86.99\% & \hfil 85.57\% \\
\cmidrule{2-7}
\centering CIFAR10, & \hfil BM & \hfil 60.08\% & \hfil 26.52\% & \hfil 8.45\% & \hfil 1.92\% &\cellcolor{yellow!60} \hfil 0.34\% \\
\cmidrule{2-7}
\centering VGG, & \hfil BL &\cellcolor{yellow!60} \hfil 52.99\% &\cellcolor{yellow!60} \hfil 18.98\% &\cellcolor{yellow!60} \hfil 5.02\% &\cellcolor{yellow!60} \hfil 1.27\% & \hfil 0.4\% \\
\cmidrule{2-7}
\hfil 91.96\% & \hfil BD & \hfil 91.18\%& \hfil 91.08\% & \hfil 91.04\% & \hfil 90.87\% & \hfil 90.68\%\\
\cmidrule{2-7}
\hfil LP & \hfil BD-F & \hfil 91.12\%& \hfil 90.93\% & \hfil 90.88\% & \hfil 90.75\% & \hfil 90.44\%\\
\cmidrule{2-7}
\hfil & \hfil ATS & \hfil 91.10\%& \hfil 90.92\% & \hfil 90.83\% & \hfil 90.61\% & \hfil 89.82\% \\
\cmidrule{2-7}
\hfil & \hfil NC  & \hfil 91.19\%& \hfil 91.18\% & \hfil 91.17\% & \hfil 91.12\% & \hfil 91.11\%\\
\midrule
\hfil & \hfil FM & \hfil 52.6\% & \hfil 37.63\% & \hfil 26.18\% & \hfil 18.59\% & \hfil 13.53\% \\
\cmidrule{2-7}
\hfil CIFAR100, & \hfil FL & \hfil 53.07\% & \hfil 38.01\% & \hfil 26.59\% & \hfil 18.62\% & \hfil 13.80\% \\
\cmidrule{2-7}
\hfil VGG, & \hfil BM  & \hfil 7.99\% & \hfil 0.15\% & \hfil 0.02\% & \hfil 0.0\% & \hfil 0.0\%  \\
\cmidrule{2-7}
\centering 69.61\% & \hfil BL & \hfil 7.12\% & \hfil 0.13\% & \hfil 0.02\% & \hfil 0.0\% & \hfil 0.0\%  \\
\cmidrule{2-7}
\hfil LP & \hfil BD & \hfil 63.9\% & \hfil 55.12\% & \hfil 45.8\% & \hfil 37.72\% & \hfil 31.19\%  \\
\cmidrule{2-7}
\hfil & \hfil BD-F & \hfil 61.47\% & \hfil 49.09\% & \hfil 37.62\% & \hfil 28.31\% & \hfil 21.91\% \\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil 22.41\% & \hfil 21.03\% & \hfil 20.66\% & \hfil 20.41\% & \hfil 20.11\% \\
\bottomrule
\end{tabular}
\newline\newline 
\caption{Adaptive testing of each metric: the first column specifies the data, model, clean accuracy, and underlying data transformations. The second column specifies which metric is used for testing. The rest of the columns are the accuracy of tests prioritized by each metric during each iteration in adaptive testing. We \colorbox{yellow!60}{highlight} the best numbers for each iteration.}\label{tab:rq3-c}
\end{center}
\end{table*}


\begin{table*}
\begin{center}
\begin{tabular}{p{5cm}p{1.9cm}p{1cm}p{1.2cm}p{1.3cm}p{1.2cm}p{1.2cm}}
\toprule
%\multicolumn{6}{c}{\centering Number of Correctly Classified Inputs} \\
%\midrule
\centering Data, Model, Accuracy, Transformations & \hfil Fitness &\hfil Iter 1 & \hfil Iter 2 & \hfil Iter 3  & \hfil Iter 4 & \hfil Iter 5  \\
\midrule
\hfil & \hfil FM & \hfil 90.21\%& \hfil 89.16\% & \hfil 88.08\% & \hfil 86.96\% & \hfil 85.56\%\\
\cmidrule{2-7}
\hfil & \hfil FL  & \hfil 90.22\%& \hfil 89.17\%& \hfil 88.1\%& \hfil 86.99\% & \hfil 85.57\% \\
\cmidrule{2-7}
\centering MNIST, & \hfil BM & \hfil 60.08\% & \hfil 26.52\% & \hfil 8.45\% & \hfil 1.92\% &\cellcolor{yellow!60} \hfil 0.34\% \\
\cmidrule{2-7}
\centering LeNet-5, & \hfil BL &\cellcolor{yellow!60} \hfil 52.99\% &\cellcolor{yellow!60} \hfil 18.98\% &\cellcolor{yellow!60} \hfil 5.02\% &\cellcolor{yellow!60} \hfil 1.27\% & \hfil 0.4\% \\
\cmidrule{2-7}
\hfil 99.01\% & \hfil BD & \hfil 35.13\%& \hfil 13.79\% & \hfil 10.95\% & \hfil 9.74\% & \hfil 8.92\%\\
\cmidrule{2-7}
\hfil Mixed & \hfil BD-F & \hfil 91.12\%& \hfil 90.93\% & \hfil 90.88\% & \hfil 90.75\% & \hfil 90.44\%\\
\cmidrule{2-7}
\hfil & \hfil ATS & \hfil 91.10\%& \hfil 90.92\% & \hfil 90.83\% & \hfil 90.61\% & \hfil 89.82\% \\
\cmidrule{2-7}
\hfil & \hfil NC  & \hfil 89.76\%& \hfil 89.06\% & \hfil 88.48\% & \hfil 88.04\% & \hfil 87.88\%\\
\midrule
\hfil & \hfil FM & \hfil 94.94\%& \hfil 94.42\% & \hfil 93.89\% & \hfil 93.20\% & \hfil 92.56\%\\
\cmidrule{2-7}
\hfil & \hfil FL  & \hfil 94.94\%& \hfil 94.43\%& \hfil 93.84\%& \hfil 93.22\% & \hfil 92.54\% \\
\cmidrule{2-7}
\centering SVHN, & \hfil BM & \hfil 82.96\% & \hfil 62.08\% & \hfil 41.74\% & \hfil 26.44\% & \hfil 16.25\% \\
\cmidrule{2-7}
\centering ResNet-9, & \hfil BL & \cellcolor{yellow!60}\hfil 76.80\% & \cellcolor{yellow!60}\hfil 50.18\% & \cellcolor{yellow!60}\hfil 30.49\% & \cellcolor{yellow!60}\hfil 17.66\% & \cellcolor{yellow!60}\hfil 9.68\% \\
\cmidrule{2-7}
\hfil 95.51\% & \hfil BD & \hfil 95.49\%& \hfil 95.49\% & \hfil 95.48\% & \hfil 95.49\% & \hfil 95.47\%\\
\cmidrule{2-7}
\hfil Mixed & \hfil BD-F & \hfil 95.48\%& \hfil 95.42\% & \hfil 95.40\% & \hfil 95.38\% & \hfil 95.32\%\\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil 95.50\%& \hfil 95.50\% & \hfil 95.47\% & \hfil 95.42\% & \hfil 95.41\%\\
\midrule
\hfil & \hfil FM & \hfil 7.98\% & \hfil 1.27\% & \hfil 0.67\% & \hfil 0.52\% & \hfil 0.51\% \\
\cmidrule{2-7}
\hfil & \hfil FL & \hfil 8.01\% & \hfil 1.28\% & \hfil 0.68\% & \hfil 0.56\% & \hfil 0.53\% \\
\cmidrule{2-7}
\hfil & \hfil BM  & \hfil 63.24\% & \hfil 39.13\% & \hfil 25.45\% & \hfil 17.98\% & \hfil 13.33\%  \\
\cmidrule{2-7}
\centering CIFAR10, & \hfil BL & \hfil 57.44\% & \hfil 28.86\% & \hfil 14.74\% & \hfil 8.52\% & \hfil 5.18\%  \\
\cmidrule{2-7}
\centering VGG, & \hfil MM & \hfil 6.99\% & \hfil 0.73\% & \cellcolor{yellow!60}\hfil 0.09\% & \cellcolor{yellow!60}\hfil 0.01\% & \cellcolor{yellow!60}\hfil 0.0\%  \\
\cmidrule{2-7}
\hfil 91.26\% & \hfil ML &\cellcolor{yellow!60} \hfil 5.21\% &\cellcolor{yellow!60} \hfil 0.68\% & \hfil 0.30\% & \hfil 0.17\% & \hfil 0.07\%  \\
\cmidrule{2-7}
\hfil Mixed & \hfil BD & \hfil 17.39\% & \hfil 9.69\% & \hfil 9.44\% & \hfil 9.45\% & \hfil 9.46\%  \\
\cmidrule{2-7}
\hfil & \hfil BD-F & \hfil 13.59\% & \hfil 5.69\% & \hfil 4.69\% & \hfil 4.36\% & \hfil 4.11\% \\
\cmidrule{2-7}
\hfil & \hfil ATS & \hfil 32.69\% & \hfil 24.1\% & \hfil 21.63\% & \hfil 20.72\% & \hfil 20.33\% \\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil 39.69\% & \hfil 38.13\% & \hfil 37.30\% & \hfil 37.04\% & \hfil 36.63\% \\
\midrule
\hfil & \hfil FM & \hfil 7.98\% & \hfil 1.27\% & \hfil 0.67\% & \hfil 0.52\% & \hfil 0.51\% \\
\cmidrule{2-7}
\hfil & \hfil FL & \hfil 8.01\% & \hfil 1.28\% & \hfil 0.68\% & \hfil 0.56\% & \hfil 0.53\% \\
\cmidrule{2-7}
\hfil & \hfil BM  & \hfil 34.86\% & \hfil 19.75\% & \hfil 12.37\% & \hfil 8.98\% & \hfil 6.06\%  \\
\cmidrule{2-7}
\centering CIFAR100, & \hfil BL & \hfil 19.78\% & \hfil 7.15\% & \hfil 3.11\% & \hfil 1.81\% & \hfil 1.02\%  \\
\cmidrule{2-7}
\centering ResNet-18, & \hfil MM & \hfil 1.55\% & \hfil 0.01\% &\cellcolor{yellow!60} \hfil 0.0\% & \cellcolor{yellow!60}\hfil 0.0\% & \cellcolor{yellow!60}\hfil 0.0\%  \\
\cmidrule{2-7}
\hfil 70.45\% & \hfil ML & \cellcolor{yellow!60}\hfil 1.21\% & \cellcolor{yellow!60}\hfil 0.0\% &\cellcolor{yellow!60} \hfil 0.0\% & \cellcolor{yellow!60}\hfil 0.0\% & \cellcolor{yellow!60}\hfil 0.0\%  \\
\cmidrule{2-7}
\hfil Mixed & \hfil BD & \hfil 7.13\% & \hfil 1.51\% & \hfil 1.08\% & \hfil 0.99\% & \hfil 0.96\%  \\
\cmidrule{2-7}
\hfil & \hfil BD-F & \hfil 6.35\% & \hfil 1.35\% & \hfil 1.01\% & \hfil 0.96\% & \hfil 0.91\% \\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil 22.41\% & \hfil 21.03\% & \hfil 20.66\% & \hfil 20.41\% & \hfil 20.11\% \\
\bottomrule
\end{tabular}
\newline\newline 
\caption{Adaptive testing of each metric: the first column specifies the data, model, clean accuracy, and underlying data transformations. The second column specifies which metric is used for testing. The rest of the columns are the accuracy of tests prioritized by each metric during each iteration in adaptive testing. We \colorbox{yellow!60}{highlight} the best numbers for each iteration.}\label{tab:rq3-c}
\end{center}
\end{table*}

==> random.tex <==
python3 main.py --experiment testing  --transformation benign --iterations 5 --adv_samples 70 --test_batch_size 1000 --transformation mixed --dataset cifar100 --model vgg --testing bd --bd_layer final

\begin{table*}
\begin{center}
\caption{Adaptive testing of each metric: the first column specifies the data, model, clean accuracy, and underlying data transformations. The second column specifies which metric is used for testing. The rest of the columns are the accuracy of tests prioritized by each metric during each iteration in adaptive testing.  We \colorbox{yellow!60}{highlight} the best numbers for each iteration.}\label{tab:rq32-c}
\begin{tabular}{p{5cm}p{1.9cm}p{1cm}p{1.2cm}p{1.3cm}p{1.2cm}p{1.2cm}}
\toprule
%\multicolumn{6}{c}{\centering Number of Correctly Classified Inputs} \\
%\midrule
\centering Data, Model, Accuracy, Transformations & \hfil Fitness &\hfil Iter 1 & \hfil Iter 2 & \hfil Iter 3  & \hfil Iter 4 & \hfil Iter 5  \\
\midrule
\hfil & \hfil FM & \hfil 10.06\%& \hfil 0.37\% & \hfil 0.0\% & \hfil 0.0\% & \hfil 0.0\%\\
\cmidrule{2-7}
\hfil & \hfil FL  &\cellcolor{yellow!60} \hfil 8.23\%& \hfil 0.07\%& \hfil 0.0\%& \hfil 0.0\% & \hfil 0.0\% \\
\cmidrule{2-7}
\centering , & \hfil BM & \hfil 33.83\% & \hfil 10.7\% & \hfil 4.82\% & \hfil 2.29\% & \hfil 1.57\% \\
\cmidrule{2-7}
\centering MNIST, & \hfil BL & \hfil 44.12\% & \hfil 14.76\% & \hfil 6.13\% & \hfil 2.84\% & \hfil 1.72\% \\
\cmidrule{2-7}
\centering LeNet-1, & \hfil MM & \hfil 44.12\% & \hfil 14.76\% & \hfil 6.13\% & \hfil 2.84\% & \hfil 1.72\% \\
\cmidrule{2-7}
\centering 97.32\%, & \hfil ML & \hfil 44.12\% & \hfil 14.76\% & \hfil 6.13\% & \hfil 2.84\% & \hfil 1.72\% \\
\cmidrule{2-7}
\hfil Mixed & \hfil BD & \hfil 28.9\%& \hfil 13.16\% & \hfil 10.08\% & \hfil 9.4\% & \hfil 8.6\%\\
\cmidrule{2-7}
\hfil  & \hfil BD-F & \hfil ???\%& \hfil 4.76\% & \hfil 2.4\% & \hfil 1.86\% & \hfil 1.57\%\\
\cmidrule{2-7}
\hfil & \hfil ATS & \hfil 34.41\%& \hfil 22.92\% & \hfil 19.78\% & \hfil 17.56\% & \hfil 16.70\%\\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil ???\%& \hfil 77.67\% & \hfil 76.26\% & \hfil 75.95\% & \hfil 75.69\% \\
\midrule
\hfil & \hfil FM & \hfil 8.17\%& \cellcolor{yellow!60}\hfil 0.11\% &\cellcolor{yellow!60} \hfil 0\% & \cellcolor{yellow!60}\hfil 0\% & \cellcolor{yellow!60}\hfil 0\%\\
\cmidrule{2-7}
\hfil & \hfil FL  &\cellcolor{yellow!60} \hfil 8.23\%& \hfil 0.07\%& \hfil 0.0\%& \hfil 0.0\% & \hfil 0.0\% \\
\cmidrule{2-7}
\centering MNIST, & \hfil BM & \hfil 33.83\% & \hfil 10.7\% & \hfil 4.82\% & \hfil 2.29\% & \hfil 1.57\% \\
\cmidrule{2-7}
\centering LeNet-5, & \hfil BL & \hfil 44.12\% & \hfil 14.76\% & \hfil 6.13\% & \hfil 2.84\% & \hfil 1.72\% \\
\cmidrule{2-7}
\hfil 99.01\% & \hfil BD & \hfil 28.9\%& \hfil 13.16\% & \hfil 10.08\% & \hfil 9.4\% & \hfil 8.6\%\\
\cmidrule{2-7}
\hfil Mixed & \hfil BD-F & \hfil ???\%& \hfil 4.76\% & \hfil 2.4\% & \hfil 1.86\% & \hfil 1.57\%\\
\cmidrule{2-7}
\hfil & \hfil ATS & \hfil 31.08\%& \hfil 21.58\% & \hfil 19.01\% & \hfil 18.17\% & \hfil 16.82\%\\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil ???\%& \hfil 77.67\% & \hfil 76.26\% & \hfil 75.95\% & \hfil 75.69\% \\
\midrule
\hfil & \hfil FM & \hfil 23.42\%& \cellcolor{yellow!60}\hfil 5.97\% &\cellcolor{yellow!60} \hfil 3.62\% & \cellcolor{yellow!60}\hfil 2.72\% & \cellcolor{yellow!60}\hfil 2.26\%\\
\cmidrule{2-7}
\hfil & \hfil FL  &\cellcolor{yellow!60} \hfil 20.8\%& \hfil 6.78\%& \hfil 4.64\%& \hfil 3.7\% & \hfil 3.11\% \\
\cmidrule{2-7}
\centering SVHN, & \hfil BM & \hfil 78.35\% & \hfil 54.19\% & \hfil 38.43\% & \hfil 30.36\% & \hfil 24.23\% \\
\cmidrule{2-7}
\centering ResNet-9, & \hfil BL & \hfil 78.75\% & \hfil 54.92\% & \hfil 39.67\% & \hfil 31.06\% & \hfil 24.54\% \\
\cmidrule{2-7}
\hfil 95.90\% & \hfil BD & \hfil 39.85\%& \hfil 22.14\% & \hfil 19.56\% & \hfil 19.61\% & \hfil 19.51\%\\
\cmidrule{2-7}
\hfil Mixed & \hfil BD-F & \hfil ???\%& \hfil 12.93\% & \hfil 10.26\% & \hfil 9.21\% & \hfil 8.39\%\\
\cmidrule{2-7}
\hfil & \hfil ATS & \hfil 30.88\%& \hfil 19.96\% & \hfil 17.83\% & \hfil 16.81\% & \hfil 16.29\%\\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil ???\%& \hfil 45.10\% & \hfil 42.47\% & \hfil 41.38\% & \hfil 40.60\% \\
\midrule
\hfil & \hfil FM & \hfil 23.42\%& \cellcolor{yellow!60}\hfil 5.97\% &\cellcolor{yellow!60} \hfil 3.62\% & \cellcolor{yellow!60}\hfil 2.72\% & \cellcolor{yellow!60}\hfil 2.26\%\\
\cmidrule{2-7}
\hfil & \hfil FL  &\cellcolor{yellow!60} \hfil 20.8\%& \hfil 6.78\%& \hfil 4.64\%& \hfil 3.7\% & \hfil 3.11\% \\
\cmidrule{2-7}
\centering SVHN, & \hfil BM & \hfil 78.35\% & \hfil 54.19\% & \hfil 38.43\% & \hfil 30.36\% & \hfil 24.23\% \\
\cmidrule{2-7}
\centering VGG, & \hfil BL & \hfil 78.75\% & \hfil 54.92\% & \hfil 39.67\% & \hfil 31.06\% & \hfil 24.54\% \\
\cmidrule{2-7}
\hfil 95.19\% & \hfil BD & \hfil 39.85\%& \hfil 22.14\% & \hfil 19.56\% & \hfil 19.61\% & \hfil 19.51\%\\
\cmidrule{2-7}
\hfil Mixed & \hfil BD-F & \hfil ???\%& \hfil 12.93\% & \hfil 10.26\% & \hfil 9.21\% & \hfil 8.39\%\\
\cmidrule{2-7}
\hfil & \hfil ATS & \hfil 33.97\%& \hfil 22.78\% & \hfil 19.80\% & \hfil 18.49\% & \hfil 17.46\%\\
\cmidrule{2-7}
\hfil & \hfil NC & \hfil ???\%& \hfil 45.10\% & \hfil 42.47\% & \hfil 41.38\% & \hfil 40.60\% \\
\bottomrule
\end{tabular}
\newline\newline 
%\caption{Adaptive testing of each metric: the first column specifies the data, model, clean accuracy, and underlying data transformations. The second column specifies which metric is used for testing. The rest of the columns are the accuracy of tests prioritized by each metric during each iteration in adaptive testing.  We \colorbox{yellow!60}{highlight} the best numbers for each iteration.}\label{tab:rq32-c1}
\end{center}
\end{table*}

%\subsection{Complete Table 2}
\begin{table*}
\begin{center}
\caption*{Table (Continued)}
\begin{tabular}{p{5cm}p{1.9cm}p{1cm}p{1.2cm}p{1.3cm}p{1.2cm}p{1.2cm}}
%\toprule
%\multicolumn{6}{c}{\centering Number of Correctly Classified Inputs} \\
%\midrule
%\centering Data, Model, Accuracy, Transformations & \hfil Fitness &\hfil Iter 1 & \hfil Iter 2 & \hfil Iter 3  & \hfil Iter 4 & \hfil Iter 5  \\
\midrule
\hfil & \hfil FM &\cellcolor{yellow!60} \hfil 8.41\% & \cellcolor{yellow!60}\hfil 1.53\% & \cellcolor{yellow!60}\hfil 0.76\% & \cellcolor{yellow!60}\hfil 0.59\% & \hfil 0.53\%  \\
\cmidrule{2-7}
\hfil & \hfil FL  &\cellcolor{yellow!60} \hfil 8.41\% & \hfil 1.55\% & \hfil 0.80\% & \hfil 0.60\% & \cellcolor{yellow!60}\hfil 0.52\%  \\
\cmidrule{2-7}
\centering CIFAR10, & \hfil BM & \hfil 71.45\% & \hfil 55.24\% & \hfil 41.98\% & \hfil 33.90\% & \hfil 27.93\%  \\
\cmidrule{2-7}
\centering ResNet-18, & \hfil BL & \hfil 72.09\% & \hfil 56.62\% & \hfil 43.96\% & \hfil 35.55\% & \hfil 30.03\%  \\
\cmidrule{2-7}
\hfil 91.26\% & \hfil BD & \hfil 19.64\% & \hfil 10.46\% & \hfil 9.07\% & \hfil 8.9\% & \hfil 8.9\%  \\
\cmidrule{2-7}
\hfil Mixed & \hfil BD-F & \hfil ???\% & \hfil 3.77\% & \hfil 2.41\% & \hfil 1.88\% & \hfil 1.68\% \\
\cmidrule{2-7}
\hfil  & \hfil ATS & \hfil 31.02\% & \hfil 20.91\% & \hfil 18.58\% & \hfil 18.06\% & \hfil 17.81\% \\
\cmidrule{2-7}
\hfil & \hfil NC  & \hfil ???\% & \hfil 37.96\% & \hfil 36.29\% & \hfil 35.59\% & \hfil 34.98\% \\
\midrule
\hfil & \hfil FM &\cellcolor{yellow!60} \hfil 8.41\% & \cellcolor{yellow!60}\hfil 1.53\% & \cellcolor{yellow!60}\hfil 0.76\% & \cellcolor{yellow!60}\hfil 0.59\% & \hfil 0.53\%  \\
\cmidrule{2-7}
\hfil & \hfil FL  &\cellcolor{yellow!60} \hfil 8.41\% & \hfil 1.55\% & \hfil 0.80\% & \hfil 0.60\% & \cellcolor{yellow!60}\hfil 0.52\%  \\
\cmidrule{2-7}
\centering CIFAR10, & \hfil BM & \hfil 71.45\% & \hfil 55.24\% & \hfil 41.98\% & \hfil 33.90\% & \hfil 27.93\%  \\
\cmidrule{2-7}
\centering VGG, & \hfil BL & \hfil 72.09\% & \hfil 56.62\% & \hfil 43.96\% & \hfil 35.55\% & \hfil 30.03\%  \\
\cmidrule{2-7}
\hfil 91.48\% & \hfil BD & \hfil 19.64\% & \hfil 10.46\% & \hfil 9.07\% & \hfil 8.9\% & \hfil 8.9\%  \\
\cmidrule{2-7}
\hfil Mixed & \hfil BD-F & \hfil ???\% & \hfil 3.77\% & \hfil 2.41\% & \hfil 1.88\% & \hfil 1.68\% \\
\cmidrule{2-7}
\hfil  & \hfil ATS & \hfil 30.83\% & \hfil 22.69\% & \hfil 20.51\% & \hfil 19.59\% & \hfil 20.01\% \\
\cmidrule{2-7}
\hfil & \hfil NC  & \hfil ???\% & \hfil 37.96\% & \hfil 36.29\% & \hfil 35.59\% & \hfil 34.98\% \\
\midrule
\hfil & \hfil FM &\cellcolor{yellow!60} \hfil 2.31\% & \hfil 0.23\% & \cellcolor{yellow!60}\hfil 0.07\% & \cellcolor{yellow!60}\hfil 0.03\% & \hfil 0.01\%  \\
\cmidrule{2-7}
\hfil CIFAR100, & \hfil FL  & \hfil 2.32\% &\cellcolor{yellow!60} \hfil 0.21\% & \cellcolor{yellow!60}\hfil 0.07\% & \cellcolor{yellow!60}\hfil 0.03\% & \cellcolor{yellow!60}\hfil 0.00\%  \\
\cmidrule{2-7}
\centering ResNet-18, & \hfil BM & \hfil 45.45\% & \hfil 30.43\% & \hfil 19.46\% & \hfil 14.48\% & \hfil 10.66\%  \\
\cmidrule{2-7}
\centering 70.45\%  & \hfil BL & \hfil 44.17\% & \hfil 30.17\% & \hfil 20.51\% & \hfil 15.18\% & \hfil 11.41\%  \\
\cmidrule{2-7}
\hfil Benign & \hfil BD & \hfil 10.91\% & \hfil 2.19\% & \hfil 1.29\% & \hfil 0.99\% & \hfil 0.96\%  \\
\cmidrule{2-7}
 & \hfil BD-F & \hfil 9.24\% & \hfil 1.87\% & \hfil 1.06\% & \hfil 0.88\% & \hfil 0.73\% \\
\cmidrule{2-7}
 & \hfil NC & \hfil 25.08\% & \hfil 20.16\% & \hfil 17.98\% & \hfil 17.02\% & \hfil 16.48\% \\
 \midrule
\hfil & \hfil FM &\cellcolor{yellow!60} \hfil 2.31\% & \hfil 0.23\% & \cellcolor{yellow!60}\hfil 0.07\% & \cellcolor{yellow!60}\hfil 0.03\% & \hfil 0.01\%  \\
\cmidrule{2-7}
\hfil CIFAR100, & \hfil FL  & \hfil 2.32\% &\cellcolor{yellow!60} \hfil 0.21\% & \cellcolor{yellow!60}\hfil 0.07\% & \cellcolor{yellow!60}\hfil 0.03\% & \cellcolor{yellow!60}\hfil 0.00\%  \\
\cmidrule{2-7}
\centering ResNet-18, & \hfil BM & \hfil 45.45\% & \hfil 30.43\% & \hfil 19.46\% & \hfil 14.48\% & \hfil 10.66\%  \\
\cmidrule{2-7}
\centering 70.45\%  & \hfil BL & \hfil 44.17\% & \hfil 30.17\% & \hfil 20.51\% & \hfil 15.18\% & \hfil 11.41\%  \\
\cmidrule{2-7}
\hfil Benign & \hfil BD & \hfil 10.91\% & \hfil 2.19\% & \hfil 1.29\% & \hfil 0.99\% & \hfil 0.96\%  \\
\cmidrule{2-7}
 & \hfil BD-F & \hfil 9.24\% & \hfil 1.87\% & \hfil 1.06\% & \hfil 0.88\% & \hfil 0.73\% \\
\cmidrule{2-7}
 & \hfil NC & \hfil 25.08\% & \hfil 20.16\% & \hfil 17.98\% & \hfil 17.02\% & \hfil 16.48\% \\
\bottomrule
\end{tabular}
\newline\newline 
\end{center}
\end{table*}

==> related.tex <==
%\section{Bridge testing practice and deep learning findings}
\section{Related Work}
In this section, we further discuss some related topics on DNN testing. In particular, we want to emphasize some discrepancies between SE practices and DL findings. This brings awareness of the gaps and hopefully can lead to bridging them.

\paragraph{Neuron activation}
One of the first DNN testing works was inspired by the code coverage in traditional software testing practice to define NC~\citep{deepxplore}. 
However, the inherent difference between software and DNN challenges the direct application of the idea from one literature to the other.
In software, execution trace usually has logical and qualitative semantics, i.e., the execution trace is decided by the logical conditions in the program. 
In contrast, the neuron activation in DNNs is quantitative, and its semantics is not as clear as in software. 
Therefore, maximizing NC does not provide clear interpretations as in traditional software.

Nonetheless, NC does provide rich information about the execution of the inputs. 
In DL society, neuron activation is referred to as \emph{feature representation}, and the researchers have exploited the information from feature representations for various purposes.
For instance, higher-level explanations about DNN behaviors can be abstracted out of feature representations, which are more user-friendly than simply inspecting neuron outputs ~\citep{tcav, ace, concept-ood}.
Moreover, ~\citep{percep-metric} illustrated that feature representations can provide an effective metric for human perceptual measurement. They defined a metric based on normalized neuron activation and found that it is strongly aligned with human judgment. This leads to the design of defense against more realistic and unseen threats~\citep{percep_defense}.



\iffalse
One of the first DNN testing works was inspired by the code coverage in traditional software testing practice and defined neuron activation coverage similarly~\citep{deepxplore}. 
However, in traditional software, execution trace usually has logical and qualitative semantics, i.e., the execution trace is decided by the logical conditions in the program. In contrast, the neuron activation in DNNs is quantitative, and its semantics is not as clear as in the traditional software. 
Therefore, maximizing NC does not provide clear interpretations as in traditional software. %In fact,~\citep{NC-meaningful} found that the image generated by this metric is not natural.

However, NC does provide rich information about the execution of the inputs. For example, because in DNNs the output of one layer is the input of the next layer, the DNN can predict the class with only the neuron activation information. This in fact motivates several works on explainability.
concept-based explanations, sparse activations, letter ticket hypothesis, etc.

The DL researchers refer to neuron activation as the \emph{feature representation} and have found that the activation information can provide an effective metric for human perceptual measurement~\citep{percep-metric}.~\citep{percep-metric} defined a metric based on the normalized neuron activation and found that it is strongly aligned with human judgment. This leads to the design of defense against more realistic and unseen threats~\citep{percep_defense}.
\fi

\iffalse
~\citep{diversity-boosting} relies on the assumption that if the neuron representation of two metamorphic inputs on an intermediate layer is very divergent, then their predictions are also likely different. While the reversed argument holds that different predictions must have divergent intermediate representations, the original assumption is not necessarily true. Especially how to measure the divergence is unclear, and this can lead to distinctive prioritization of inputs. However, similar ideas in DL communities are used to design OOD detectors.

As a result, from the OOD detection perspective, the NAC maximization generates inputs whose feature representations deviate from the training data and should be treated as OOD inputs. This is consistent with the finding in~\citep{NC-meaningful} that the inputs from maximizing the NAC score are not natural. However, we need to define what bugs are a priori to handle OOD inputs.

%All of these DL findings indicate that even though maximizing the neuron activation might not be a meaningful metric for testing, using 
\fi

%~\citep{diversity-boosting} relies on the assumption that if the neuron representation of two metamorphic inputs on an intermediate layer is very divergent, then their predictions are also likely different. 
%However, this argument is not always valid. %For instance,~\citep{NC-meaningful} demonstrates that the inputs generated to maximize NAC are unnatural. 
%While the reversed argument that different predictions must have divergent intermediate representations is a logically valid, the %common assumption in DL communities.
~\citep{diversity-boosting} relies on the assumption that if the neuron representation of two metamorphic inputs on an intermediate layer is very divergent, then their predictions are also likely different. While the reversed argument always holds that different predictions must have divergent intermediate representations, the original assumption is not necessarily true. Especially how to measure the difference is unclear when the divergence is subtle, and this can lead to distinctive prioritization of inputs as in the $\ell_p$-transformation evaluations. However, similar ideas in DL communities are used to design OOD detectors. %We point the readers to an actively-studied area in DL based on this reversed argument: out-of-distribution (OOD) detection. 
OOD tests are inputs that are far from the distribution the DNN has seen during the training (i.e., in-distribution), hence it is undefined behavior for DNN to predict given those tests.
Assuming that in-distribution and OOD inputs have distinctive feature attribution patterns, there have been various approaches to exploiting statistical information from feature representations to distinguish in-distribution vs. OOD inputs~\citep{ood-mahalanobis,ood-jtla}, and understand the characteristics of OOD inputs~\citep{concept-ood}.
Consequently, bringing the OOD detection perspective to DNN testing, we suggest that the NC maximization would make the feature representations of generated inputs deviate from the training data, which are actually OOD.
This is consistent with the finding in~\citep{NC-meaningful} that the inputs from maximizing the NC score are not natural. 
To this end, one needs to define the scope of bugs a priori to avoid unnecessary execution against OOD inputs. %, and design the measure of divergence accordingly.
%\jc{@Zi: please check}

\paragraph{Gradient}
We carefully analyzed the application of gradients in DL testing. Gradients naturally exist for many mathematical functions, including neural networks. They quantify the local variability of a function and can provide the optimal linear approximation in a small neighborhood. Our gradient-based metrics are the applications of linear approximation and some of them coincide with the adversarial attack algorithms in DL literature, which indicates that these algorithms can be viewed as concrete instantiations of our framework for small additive transformations. Because traditional software is mostly not differentiable, gradients are less often used in software testing works. However, the gradient-based methods have been successful in many DL applications, encompassing $\ell_p$-adversarial attacks and gradient-based explanations~\citep{LIME, integrated-gradient}. We believe that the SE practice can also utilize gradients as tools for testing DNNs, such as recent works on numerical defects in DL programs~\citep{grist,reliability}.

%Similar to neuron activation, gradients also encode rich information on the properties of DNNs. Gradient-based explanations~\zw{Jihye}

\paragraph{Bugs}In this work, we restrict our scope to functionality bugs, i.e., inputs that are misclassified according to human perception. However, DL bugs can manifest in various forms. In~\citep{debug}, the authors categorize model bugs into three types: model contamination, data contamination, and test-time contamination. Model contamination is caused by errors in the model parameters, for example, incorrectly initialized parameters; data contamination comes from defects in the training data; and test-time contamination is caused by shifts in test data.  
Functionality bugs can be viewed as test-time contamination: our data are transformed at test time. However, there are many more types of bugs in the DL system to be addressed and SE techniques can be applied. For example, model contamination is often caused by API misuses, which has been studied in many SE works~\citep{api-misuse1,api-misuse2}.
 
\paragraph{Diversity}
We claim that merely increasing diversity is not the ideal framework for DNN functionality testing. However, we do not claim that diversity is useless for DL testing. It depends on our testing goal. A natural diversity issue of DL systems is fairness and bias~\citep{fairness,nn-bias}: Between subgroups, DL systems contain performance discrepancies and make biased decisions towards a certain subgroup. This would also cause concerns for the deployment of DL systems because DNN classifications can discriminate certain subgroups. If the tests were only from a subgroup, then potential fairness and bias issues would be concealed. Therefore, designing meaningful diversity measures can help expose and alleviate the bias and fairness issues in DL systems.

%With these DL lessons, a natural question arises:
%\begin{tcolorbox}
%  What should be treated as bugs for DL systems?  
%\end{tcolorbox}
%We leave this as an open problem. We believe that if bugs are defined properly, then directed testing is more effective to detect the bugs.
